Deep Functional Factor Models: Forecasting High-Dimensional Functional Time Series via Bayesian Nonparametric Factorization

This paper introduces the Deep Functional Factor Model (DF2M), a Bayesian nonparametric model designed for analysis of high-dimensional functional time series. DF2M is built upon the Indian Buffet Process and the multi-task Gaussian Process, incorporating a deep kernel function that captures non-Markovian and nonlinear temporal dynamics. Unlike many black-box deep learning models, DF2M offers an explainable approach to utilizing neural networks by constructing a factor model and integrating deep neural networks within the kernel function. Additionally, we develop a computationally efficient variational inference algorithm to infer DF2M. Empirical results from four real-world datasets demonstrate that DF2M provides better explainability and superior predictive accuracy compared to conventional deep learning models for high-dimensional functional time series.

==> tables/table1.tex <==
\resizebox{0.95\linewidth}{!}{ \setlength{\tabcolsep}{2.5pt}
\begin{tabular}{lccc@{\hspace{10pt}}lc@{\hspace{10pt}}cc@{\hspace{10pt}}cc@{\hspace{10pt}}cc@{\hspace{10pt}}cc@{\hspace{10pt}}cc@{\hspace{10pt}}cc}
    \toprule
    & \multirow{2}{*}{$h$} & \multicolumn{2}{c}{{\scriptsize DF\textsuperscript{2}M-LIN}} & \multicolumn{2}{c}{{\scriptsize LIN}}  & \multicolumn{2}{c}{{\scriptsize DF\textsuperscript{2}M-LSTM}} & \multicolumn{2}{c}{{\scriptsize LSTM}} & \multicolumn{2}{c}{{\scriptsize DF\textsuperscript{2}M-GRU}} &  \multicolumn{2}{c}{{\scriptsize GRU}} & \multicolumn{2}{c}{{\scriptsize DF\textsuperscript{2}M-ATTN}} &  \multicolumn{2}{c}{{\scriptsize ATTN}}  \\
    \cmidrule(l{5pt}r{10pt}){3-4} \cmidrule(l{2pt}r{10pt}){5-6} \cmidrule(l{2pt}r{10pt}){7-8} \cmidrule(l{2pt}r{10pt}){9-10} \cmidrule(l{2pt}r{10pt}){11-12} \cmidrule(l{2pt}r{10pt}){13-14} \cmidrule(l{2pt}r{10pt}){15-16} \cmidrule(l{2pt}r{3pt}){17-18}
    &     & {\scriptsize MSPE}   & {\scriptsize MAPE}   & {\scriptsize MSPE}   & {\scriptsize MAPE}   & {\scriptsize MSPE}  & {\scriptsize MAPE}   & {\scriptsize MSPE}  & {\scriptsize MAPE}   & {\scriptsize MSPE}  & {\scriptsize MAPE}  & {\scriptsize MSPE}  & {\scriptsize MAPE}   & {\scriptsize MSPE}  & {\scriptsize MAPE}   & {\scriptsize MSPE}  & {\scriptsize MAPE}  \\
\midrule\multirow{3}{*}{\rotatebox{90}{\parbox{1.5cm}{\raggedleft{\tiny\textbf{\textit{\  Japanese\\ \ Mortality}}}}}} & 1 & 4.707 & 1.539 & 7.808 & 2.092 & 3.753 & 1.205 & 4.989 & 1.447 & 4.092 & 1.318 & 8.800 & 1.691 & \textbf{3.608} &  \textbf{1.119} & 13.44 & 3.166 \\
 & 2 & 4.567 & 1.446 & 8.774 & 2.227 & 4.164 & 1.322 & 5.597 & 1.523 & 4.395 & 1.402 & 8.552 & 1.809 & \textbf{3.839} & \textbf{1.203} & 14.85 & 3.363 \\
 & 3 & 5.623 & 1.635 & 9.228 & 2.313 & 4.513 & 1.427 & 6.501 & 1.684 & 4.898 & 1.537 & 10.41 & 1.865 & \textbf{3.985} & \textbf{1.264} & 16.17 & 3.546 \\
\midrule\multirow{3}{*}{\rotatebox{90}{\parbox{1.5cm}{\centering{\tiny\textbf{\textit{\quad\quad Energy\\\quad\quad Consm.}}}}}} & 1 & 10.29 & 2.334 & 16.16 & 2.939 & \textbf{8.928} & \textbf{2.176} & 13.51 & 2.635 & 9.132 & 2.204 & 15.55 & 2.872 & 14.22 & 2.741 & 17.03 & 3.130 \\
 & 2 & 17.58 & 3.060 & 18.95 & 3.214 & \textbf{11.60} & \textbf{2.478} & 19.71 & 3.278 & 15.49 & 2.801 & 24.02 & 3.518 & 18.70 & 3.141 & 17.79 & 3.216 \\
 & 3 & 17.64 & 3.100 & 20.27 & 3.342 & 17.26 & 3.063 & 24.61 & 3.759 & \textbf{14.13} & \textbf{2.801} & 23.91 & 3.626 & 19.03 & 3.163 & 18.24 & 3.268 \\
\midrule\multirow{3}{*}{\rotatebox{90}{\parbox{1.5cm}{\raggedleft{\tiny\textbf{\textit{\quad\quad Global\\ Mortality}}}}}} & 1 & 10.78 & 2.319 & 16.84 & 2.783 & \textbf{7.672} & \textbf{1.726} & 13.28 & 2.332 & 8.741 & 1.967 & 14.12 & 2.211 & 9.905 & 2.141 & 39.52 & 5.332 \\
 & 2 & 9.300 & 2.041 & 18.05 & 2.949 & \textbf{8.088} & \textbf{1.823} & 16.29 & 2.572 & 8.714 & 1.951 & 15.33 & 2.403 & 10.46 & 2.237 & 41.83 & 5.506 \\
 & 3 & 9.706 & 2.106 & 19.93 & 3.174 & \textbf{8.954} & \textbf{1.978} & 17.08 & 2.680 & 9.730 & 2.110 & 17.53 & 2.597 & 11.12 & 2.324 & 43.95 & 5.643 \\
\midrule\multirow{3}{*}{\rotatebox{90}{\parbox{1.5cm}{\raggedleft{\tiny\textbf{\textit{\quad\quad Stock\\ Intraday}}}}}} & 1 & \textbf{99.58} & \textbf{6.424} & 137.5 & 7.896 & 107.5 & 6.741 & 193.3 & 9.281 & 102.5 & 6.675 & 414.0 & 14.12 & 104.2 & 6.695 & 103.4 & 6.579 \\
 & 2 & 101.2 & 6.505 & 127.8 & 7.491 & 118.8 & 7.141 & 176.0 & 9.283 & 117.3 & 7.339 & 445.9 & 14.66 & 103.4 & 6.646 & \textbf{98.39} & \textbf{6.392} \\
 & 3 & \textbf{89.82} & \textbf{6.269} & 139.1 & 7.924 & 113.6 & 7.294 & 213.8 & 10.20 & 95.49 & 6.649 & 427.2 & 14.07 & 93.93 & 6.427 & 91.21 & 6.275 \\
\bottomrule
\vspace{-20pt}
\end{tabular} }

==> tables/table1_transpose.tex <==
\resizebox{0.95\linewidth}{!}{ 
    \setlength{\tabcolsep}{2.5pt}
    \begin{tabular}{lcccccccccccccccc}
    \toprule
    & & \multicolumn{3}{c}{{\scriptsize Japanese Mortality}} & \multicolumn{3}{c}{{\scriptsize Energy Consumption}} & \multicolumn{3}{c}{{\scriptsize Global Mortality}} & \multicolumn{3}{c}{{\scriptsize Stock Intraday }} \\
    \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}
   $h$ &  & 1 & 2 & 3 & 1 & 2 & 3 & 1 & 2 & 3 & 1 & 2 & 3& \\
    \midrule
   
  
  
    \midrule
    {\scriptsize MSPE} & &  \\
    {\scriptsize MAPE} & &  \\
    \midrule
    {\scriptsize MSPE} & & \\
    {\scriptsize MAPE} & &  \\
    \midrule
    {\scriptsize MSPE} & &  \\
    {\scriptsize MAPE} & &  \\
    \midrule
    {\scriptsize MSPE} & &  \\
    {\scriptsize MAPE} & &  \\
    \midrule
    {\scriptsize MSPE} & &  \\
    {\scriptsize MAPE} & &  \\
    \bottomrule
    \end{tabular}
}    
